Passive Optical Networking for 5G and Beyond 5G Low-Latency Mobile Fronthauling Services

Passive optical network (PON) technology offers an attractive cost-efficient alternative to support 5G and Beyond 5G mobile network fronthauling (MFH). However, MFH for such networks is challenging given its high bandwidth and strict latency requirements. To reduce these requirements, radio access network (RAN) functional splitting has been introduced in 5G networks; this provides more flexibility in resource allocation since the protocol stack is distributed between the centralized and the distributed units. In contrast to the conventional MFH requirement of the RF-PHY splitting, the MFH traffic produced by higher-layer splittings becomes more dependent on the actual user traffic load. By capitalizing on the new characteristics of the MFH traffic with RAN functional splitting, this article introduces a resource allocation mechanism to improve the performance of PONs serving MFH.

==> alg.tex <==
\begin{algorithm}[!t]

 %\small

    \caption{\BS Multi-ONU Customer Support \acs{DWBA} Algorithm}
    \label{alg:gs-ipact}
\SetAlgoLined


\SetKwInput{KwIni}{}
% \KwIni{$\mathcal{R}_{l} \leftarrow \emptyset, \forall l \in \mathcal{G}$}
\KwIni{$\mathcal{R}_{i} \leftarrow \emptyset, \forall i \in \mathcal{O}$}

    \For{each received report R from \ac{ONU} i in cycle j}{ 

        \If{ONU $i \in \mathcal{O}$}{
        
        
            \eIf{ $\left\vert{\mathcal{R}_{fl}}\right\vert$ > $0$}
            {%else
                
                 $Granted^{fl}_{i}  \leftarrow \hspace{0.1cm}  BandwidthSlicing()$
                
              
            
            }{
            
              $Granted^{fl}_{i} \leftarrow \hspace{0.1cm}  \left\big(0,0,0\right\big)$
            
            } 
        
             $Granted^{fl}_{i}  \leftarrow \hspace{0.1cm}  BandwidthAllocation()$
            
            $Gate^{j}_{i} =  (Granted^{ds}_{i},  Granted^{fl}_{i})$
            
            
            
            
            Send $Gate^{j}_{i}$
            

        }
       
        }
       %\mathcal{R}_k \leftarrow \emptyset
   
  \SetKwFunction{FMain}{\textbf{BandwidthSlicing}}
    \SetKwProg{Fn}{}{}{}
    \Fn{\FMain{}}{


         $w^{fl}_{i} = min(\left\vert{\mathcal{R}_{fl}}\right\vert$,  $\theta\cdot Z $)

        Calculate $f^{fl}_{i}$ based on \ac{TWDM}-scheduler 
    
        Calculate  $t^{fl}_{i}$
    
    %   \textbf{return}  $\left\big(f^{fl}_{i},w^{fl}_{i},t^{fl}_{i}\right\big)$
 }
\textbf{\textbf{return}  $\left\big(f^{fl}_{i},w^{fl}_{i},t^{fl}_{i}\right\big)$}

  

  \SetKwFunction{FMain}{\textbf{BandwidthAllocation}}
    \SetKwProg{Fn}{}{}{}
    \Fn{\FMain{}}{


        $w^{ds}_{i} = min(\left\vert{\mathcal{R}_{ds}}\right\vert$, w^{max}_i)
        %calculate w according to the limited policy
            
        Calculate  $f^{ds}_{i}$ based on \ac{TWDM}-scheduler 
  
        Calculate  $t^{ds}_{i}$
    
    %   \textbf{return}  $\left\big(f^{ds}_{i},w^{ds}_{i},t^{ds}_{i}\right\big)$
 }
\textbf{\textbf{return}  $\left\big(f^{ds}_{i},w^{ds}_{i},t^{ds}_{i}\right\big)$}

\end{algorithm}
